A Grand Scan of the pMSSM Parameter Space for Snowmass 2021

We present a flexible framework for interpretation of SUSY sensitivity studies for future colliders in terms of the phenomenological minimal supersymmetric standard model (pMSSM). We perform a grand scan of the pMSSM 19-dimensional parameter space that covers the accessible ranges of many collider scenarios, including electron, muon, and hadron colliders at a variety of center of mass energies. This enables comparisons of sensitivity and complementarity across different future experiments, including both colliders and precision measurements in the Cosmological and Rare Frontiers. The details of the scan framework are discussed, and the impact of future precision measurements on Higgs couplings, the anomalous muon magnetic moment, and dark matter quantities is presented. The next steps for this ongoing effort include performing studies with simulated events in order to quantitatively assess the sensitivity of selected future colliders in the context of the pMSSM.

==> sections/interpretation/interpretation.tex <==
\section{Summarizing the kinematics of non-excluded pMSSM models}
\label{sec:interpretation}

Models resulting from a pMSSM scan and that have not been excluded by experimental results can be used to identify new promising regions in experimental observable space (the space made up of all experimental observables, such as momenta of particles and invariant masses of combinations of particles) which can be studied to develop future BSM searches and even guide future experimental design. Non-excluded models were explored in previous ATLAS and CMS searches \htr{WH: not sure if I should cite the ATLAS and CMS results again} to understand why they evaded the reach of these experiments. Within ATLAS, some of these models had their mass spectra manually inspected to gain insight into their expected signature in experimental observable space. However, the experimental observable space of the non-excluded models was not systematically probed and no new searches were designed on the basis of the non-excluded models, owing to the difficulty of interpreting thousands of models manually. CMS interpreted the non-excluded models as a function of average values of observables. This yielded valuable information about the observables of non-excluded models, but was difficult to interpret because of the large number of models. 

Systematically probing the observable space of non-excluded models requires novel techniques that are able to summarize thousands of models that populate high-dimensional observable spaces. Machine learning (ML) is especially adept at processing high-dimensional spaces and can be utilized to identify promising new search regions inspired by the pMSSM. In particular, ML clustering techniques, which group similar data points together, could group multiple models with different theory parameters but similar experimental signatures, forming the basis for new search regions (since the regions are based on models that have evaded previous searches). A sketch of the proposed clustering workflow is shown in Figure~\ref{fig:clusteringWorkflow}. Once a set of regions has been selected, further studies can be performed to assess the viability of robustly estimating SM backgrounds for these regions with (semi)-data-driven methods. (These studies would address questions such as the following: Can a control region with sufficient data statistics be designed?)

\begin{figure}[!htbp]
  \centering
  \subfloat[Theory parameter space]{
    \includegraphics[width=0.313\textwidth]{sections/interpretation/plots/theorySpace.pdf}
  }
  \subfloat[Observable space]{
    \includegraphics[width=0.313\textwidth]{sections/interpretation/plots/expSpace.pdf}
  }
  \subfloat[Clustering-produced regions]{
    \includegraphics[width=0.313\textwidth]{sections/interpretation/plots/searchSpace.pdf}
  }
  
  \caption{Workflow for interpreting non-excluded pMSSM models with clustering in a toy example two-dimensional space. The two theory parameter values for four models (SM, pMSSM1-3) are shown in (a), while the space that these models populate in experimental observable space (filled with MC simulations of the models) is shown in (b) and (c).
  }
  \label{fig:clusteringWorkflow}
\end{figure}

Several techniques, such as $k$-means~\cite{kmeans} and density-based clustering~\cite{dbscan}, exist that can be used to group models with similar experimental signatures together. 
Feasibility studies were performed which were based on SMS searches for new physics in events with two top quarks and significant missing transverse energy in the all-hadronic channel. The simplified model has two parameters, the top squark mass ($m_{\tilde{t}}$) and the neutralino mass ($m_{\tilde{\chi}^0}$), which have a known effect on the observable space. A five-dimensional observable space, consisting of common variables used in analyses (i.e., MET, HT, $p_{\mathrm{T}}$'s of the leading four jets, and jet multiplicity), was clustered using the $k$-means+gap statistic~\cite{Tibishirani} method. Additionally, simulations of a grid of SMS models with different theory parameter values, expected to be associated with distinct distributions of their observables, were produces using Madgraph+Delphes. The results of applying $k$-means to form clusters of this theory model grid in the two-dimensional theory parameter space are shown in Figure~\ref{fig:stopClustering}a and demonstrate that $k$-means groups models in a similar way as the manually designed search (which had three major regions~\cite{stop0L_3}). The exact number of clusters (i.e., regions) is not important, since the final goal of the approach is to reduce thousands of models to a handful of promising regions. Similar to the visualization used in the Run~1 CMS pMSSM scan, Figure~\ref{fig:stopClustering}b shows the median and 68\% confidence interval (CI) of the observables used for clustering for each of the clusters. Figure~\ref{fig:stopClustering}b could have included all the SMS models but this would have been more difficult to interpret and would yield less insight into what type of regions could be designed to be sensitive to non-excluded models. The reduction from 100s of SMS models to three regions significantly helps the interpretability of the kinematics of the non-excluded models. Figure~\ref{fig:stopClustering}b also shows 

\begin{figure}[ht]
  \centering \subfloat[]{\includegraphics[width=0.45\textwidth]{sections/interpretation/plots/grid_postclustering_k3_MET_HT_pT_1jet_pT_2jet_pT_3jet_pT_4jet_nj_good_gap.pdf}}
  \subfloat[]{\includegraphics[width=0.39\textwidth]{sections/interpretation/plots/obs_cms_style_ttMET_postclustering_k3_MET_HT_pT_1jet_pT_2jet_pT_3jet_pT_4jet_nj_good_gap}}
  \caption{\label{fig:stopClustering} Division of a SMS model grid (a) after applying $k$-means on common observables. The median and 68\% CI bands of observables are shown in (b) which indicates that the leading difference for these models is the MET and jet multiplicity, as expected. The green dots correspond to a region where the sparticle masses are similar and thus only low-\pt\ objects are produced which results in a low jet multiplicity. The red dots, on the other hand, are have large sparticle mass splittings which results in large MET. The y-axis of (b) is the value of the observable after being normalized to be in a range of [0,1].}
\end{figure}

Applying the above clustering technique to pMSSM scans which include future experiments and colliders could guide detector and trigger design by identifying regions of observable space that are populated by pMSSM models but for which a proposed analysis, trigger, or detector designs have limited sensitivity.

==> sections/mcmc/tables/measurements.tex <==
\begin{table}[!htp]
\begin{center}
\begin{tabular}{lll}
Observable & Measurement  \\
\hline
%https://pdg.lbl.gov/2020/listings/rpp2020-list-B-plus-minus.pdf                    
$BR(B\rightarrow\tau\nu)$ & $(1.09 \pm 0.24)\times 10^{-4}$  \\ 
%https://pdg.lbl.gov/2020/listings/rpp2020-list-D-star-2010-plus-minus.pdf          
$BR(D_s\rightarrow\tau\nu)$ & $(5.48 \pm 0.23)\times 10^{-2}$  \\     
$BR(D_s\rightarrow \mu\nu)$ & $(5.49 \pm 0.16)\times 10^{-3}$  \\
\hline
\end{tabular}
\caption{Experimental results with Gaussian contributions to the McMC likelihood, from the Particle Data Group \cite{Zyla:2020zbs}.}
\label{tab:measurements}
\end{center}
\end{table}





